Measurement of the Mass Difference m(B0) - m(B+)

Using 230 million B Bbar events recorded with the BABAR detector at the e+ e- storage rings PEP-II, we reconstruct approximately 4100 B0 to J/psi K+ pi- and 9930 B+ to J/psi K+ decays with J/psi to mu+ mu- and e+ e-. From the measured B-momentum distributions in the e+ e- rest frame, we determine the mass difference m(B0) - m(B+) = (+0.33 +- 0.05 +- 0.03) MeV/c^2.

==> abstract.tex <==
\begin{abstract}

Using $230\times 10^6$ $B\bar{B}$ events recorded with the {BABAR} detector at
the $e^+e^-$ storage rings {PEP-II}, we reconstruct approximately 4100
$B^0\rightarrow J/\psi K^+\pi^-$ and 9930 $B^+\rightarrow J/\psi K^+$ decays
with $J/\psi\rightarrow\mu^+\mu^-$ and $e^+e^-$. From the measured $B$-momentum
distributions in the $e^+e^-$ rest frame, we determine the mass difference
$m(B^0)-m(B^+)=(+0.33\pm 0.05\pm 0.03)\,\mathrm{MeV}\!/c^2$.

\end{abstract}

